ShapeLLM: Universal 3D Object Understanding for Embodied Interaction

This paper presents ShapeLLM, the first 3D Multimodal Large Language Model (LLM) designed for embodied interaction, exploring a universal 3D object understanding with 3D point clouds and languages. ShapeLLM is built upon an improved 3D encoder by extending ReCon to ReCon++ that benefits from multi-view image distillation for enhanced geometry understanding. By utilizing ReCon++ as the 3D point cloud input encoder for LLMs, ShapeLLM is trained on constructed instruction-following data and tested on our newly human-curated benchmark, 3D MM-Vet. ReCon++ and ShapeLLM achieve state-of-the-art performance in 3D geometry understanding and language-unified 3D interaction tasks, such as embodied visual grounding. Project page: https://qizekun.github.io/shapellm/

==> fig/cat_pie.tex <==
\begin{figure}[h!]
\centering
\includegraphics[width=0.8\linewidth]{fig/src/cat_pie.pdf}
\vspace{-5pt}
\captionof{figure}{\textbf{Ablation study on visual prompt number}. The performance of \shapellm\ on 3D MM-Vet is reported.
}
\label{fig:number_prompts}
\end{figure}

==> fig/joint_vis_ovpart.tex <==
\begin{figure}[t!]
  \centering
  \subfloat[\textbf{Visualization of multi-view query results.} The distinct colors serve to denote distinct image queries.]{\includegraphics[width=0.38\textwidth]{fig/src/query.pdf}\label{fig:query}}
  \hfill
  \subfloat[\textbf{Part understanding examples} of unseen objects.]{\includegraphics[width=0.58\textwidth]{fig/src/vis.pdf}\label{fig:ov_part}}
  \caption{Visualization of the learned multi-view query and part understanding examples.}
  \label{fig:combined}
\vspace{-10pt}
\end{figure}


==> fig/mmvet.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.99\linewidth]{fig/src/mmvet.pdf}
\vspace{-3pt}
\captionof{figure}{\textbf{3D MM-Vet dataset sample.} A wealth of precise evaluation metrics enable a comprehensive assessment.
}
\vspace{-18pt}
\label{fig:mmvet}
\end{figure}


==> fig/prompt.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=0.98\linewidth]{fig/src/gpt4v.pdf}
\vspace{-5pt}
\captionof{figure}{\textbf{Construction illustration of instruct-following data using GPT-4V~\cite{GPT4Vision23}.} Four perspective views are input into GPT-4V. In-context prompts focusing on different topics are explicitly incorporated to ensure data diversity.
}\label{fig:prompt}
\vspace{-15pt}
\end{figure}



==> fig/vis.tex <==
\begin{figure}[t!]
\centering
\includegraphics[width=\linewidth]{fig/src/vis.pdf}
\vspace{-20pt}
\captionof{figure}{\textbf{Part understanding examples} of unseen objects.
}\label{fig:ov_part}
\vspace{-10pt}
\end{figure}

==> tab/cls/3dmmvet-c.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{3pt}
  \caption{\textbf{Zero-shot 3D multimodal comprehension} of \textit{robustness} on 3D MM-Vet-C. \textbf{\texttt{Clean}}: no corruptions. \textbf{\texttt{Single-View}}: randomly select a camera viewpoint within the unit sphere and generate a \textbf{single viewpoint} within the FoV on polar coordinates. \textbf{\texttt{Jitter}}: Gaussian jittering with noise $\epsilon\sim\mathcal{N}(0,\sigma^2)$ and $\sigma=0.01$.
  \textbf{\texttt{Rotate}}: random SO(3) rotation sampling over X-Y-Z Euler angle $(\alpha,\beta,\gamma)\sim \mathcal{U}(-\theta,\theta)$ and $\theta=\pi/6$.
  }
  \label{tab:mmvetc}
  \vspace{-8pt}
  \centering
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccc}
    \toprule[0.95pt]
        \multirow{2}{*}[-0.5ex]{Method} & \multicolumn{4}{c}{\textbf{3D MM-Vet-C Variants}}\\
        \cmidrule(lr){2-5}
        & \textbf{\texttt{Clean}} & \textbf{\texttt{Single}}-\textbf{\texttt{View}} & \textbf{\texttt{Jitter}} & \textbf{\texttt{Rotate}}\\ 
        \midrule[0.6pt]
        PointBind\&LLM~\cite{pointbind23} & 23.5 & 20.4 & 19.7 & 19.5\\
        PointLLM-7B~\cite{pointllm23} & 41.2 & 33.6 & 38.8 & 40.6\\
        PointLLM-13B~\cite{pointllm23} & 46.6 & 41.3 & 42.3 & 44.2\\
        \rowcolor{linecolor4}\textbf{\shapellm-7B} & \textbf{47.4} & \textbf{38.3} & \textbf{45.8} & \textbf{42.7}\\
        \rowcolor{linecolor3}\textbf{\shapellm-13B} & \textbf{53.1} & \textbf{43.6} & \textbf{47.8} & \textbf{49.3}\\
        \bottomrule[0.95pt]
    \end{tabular}
    % }
% \vspace{-15pt}
\end{table}

==> tab/cls/3dmmvet.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{6pt}
  \caption{\textbf{Zero-shot 3D multimodal comprehension evaluation} of \textit{core VL capabilities in 3D context} on 3D MM-Vet.
  \textbf{\texttt{Rec}}: General Visual Recognition, \textbf{\texttt{Know}}: Knowledge, \textbf{\texttt{Gen}}: Language Generation, \textbf{\texttt{Spat}}: Spatial Awareness, \textbf{\texttt{Emb}}: Embodied Interaction.
  }
  \label{tab:mmvet}
  \vspace{-5pt}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule[0.95pt]
        Method & \textbf{\texttt{Rec}} & \textbf{\texttt{Know}} & \textbf{\texttt{Gen}} & \textbf{\texttt{Spat}} & \textbf{\texttt{Emb}} & Total  \\ 
        \midrule[0.6pt]
         Point-Bind\&LLM \citep{pointbind23} & 11.3 & 11.6 & 34.2 & 22.2 & 31.9 & 20.0 \\
        PointLLM-7B~\citep{pointllm23} & 40.6 & 49.5 & 34.3 & 29.1 & 48.7 & 41.2 \\
        PointLLM-13B~\citep{pointllm23} & 46.6 & 48.3 & 38.8 & 45.2 & 50.9 & 46.6 \\
        \rowcolor{linecolor4}\textbf{\shapellm-7B} & \textbf{36.5} & \textbf{35.1} & \textbf{36.9} & \textbf{35.1} & \textbf{52.5} & \textbf{39.0}\\
        \rowcolor{linecolor3}\textbf{\shapellm-13B} & \textbf{46.8} & \textbf{53.0} & \textbf{53.9} & \textbf{45.3} & \textbf{68.4} & \textbf{53.1}\\
        \bottomrule[0.95pt]
    \end{tabular}
    }
\end{table}

==> tab/cls/caption.tex <==
\begin{table}[h!]
\centering
\caption{\textbf{3D object captioning results on Objaverse.} Models are evaluated using human evaluation, GPT-4 evaluation, and traditional metrics. A primary focus is placed on human and GPT-4 evaluation, along with data-driven metrics (Sentence-BERT and SimCSE).}
\label{tab:object_captioning}
\resizebox{\linewidth}{!}{

\begin{tabular}{lccccccccc}
\toprule
Model & Correctness & Hallucination$\downarrow$ & Precision & GPT-4 & Sentence-BERT & SimCSE & BLEU-1 & ROUGE-L & METEOR \\ \midrule
InstructBLIP-7B & 2.56 & 0.77 & 76.99 & 45.34 & 47.41 & 48.48 & 4.27 & 8.28 & 12.99 \\
InstructBLIP-13B & 2.58 & 1.13 & 69.56 & 44.97 & 45.90 & 48.86 & 4.65 & 8.85 & 13.23 \\
LLaVA-7B & 2.76 & 0.86 & 76.30 & 46.71 & 45.61 & 47.10 & 3.64 & 7.70 & 12.14 \\
LLaVA-13B & 2.43 & 0.86 & 73.97 & 38.28 & 46.37 & 45.90 & 4.02 & 8.15 & 12.58 \\ \midrule
3D-LLM & 1.77 & 1.16 & 60.39 & 33.42 & 44.48 & 43.68 & 16.91 & 19.48 & 19.73 \\
PointLLM-7B & 3.04 & 0.66 & \textbf{82.14} & 44.85 & 47.47 & 48.55 & 3.87 & 7.30 & 11.92 \\
PointLLM-13B & 3.10 & 0.84 & 78.75 & 48.15 & 47.91 & 49.12 & 3.83 & 7.23 & 12.26 \\ 
\textbf{ShapeLLM-7B} & - & \textbf{-} & \textbf{-} & - &- & - & - & - & - \\
\textbf{PointLLM-13B} & \textbf{-} & - & - & \textbf{-} & \textbf{-} & \textbf{-} & - & - & - \\ \midrule
Human & 2.67 & 0.22 & 92.46 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 & 100.00 \\ 
\bottomrule
\end{tabular}
}
\end{table}

==> tab/cls/generative_cls.tex <==
\begin{table}[h!]
\centering
\caption{\textbf{Generative 3D object classification results on the \textbf{M}odelNet40 test split and \textbf{O}bjaverse.} The results show the classification accuracy under the \textbf{I}nstruction-typed (I) prompt ``What is this?" and the \textbf{C}ompletion-typed (C) prompt ``This is an object of ".}
\label{tab:generative_classification}
\resizebox{\linewidth}{!}{

\begin{tabular}{@{}l@{\hspace{0.5em}}c@{\hspace{0.5em}}ccccc}
\toprule
Model & Input & ModelNet40 (I) & ModelNet40 (C) & Objaverse (I) & Objaverse (C) & Average \\ \midrule
InstructBLIP-7B & Single-V. Img. & 19.53 & 31.48 & 45.00 & 42.00 & 34.50 \\
InstructBLIP-13B & Single-V. Img. & 25.97 & 31.40 & 37.00 & 31.50 & 31.47 \\
LLaVA-7B & Single-V. Img. & 39.75 & 39.67 & 49.50 & 50.50 & 44.86 \\
LLaVA-13B & Single-V. Img. & 37.12 & 36.06 & 53.00 & 50.50 & 44.17 \\ \midrule
3D-LLM & 3D Obj. + Mul.-V. Img. & - & - & 49.00 & 41.50 & 45.25 \\
Point Bind\&LLM & 3D Point Cloud & 51.90 & 39.71 & 6.00 & 4.50 & 25.53 \\
PointLLM-7B & 3D Point Cloud & 53.44 & 51.82 & 55.00 & 51.00 & 52.82 \\
PointLLM-13B & 3D Point Cloud & 53.00 & 52.55 & 56.50 & 51.50 & 53.39 \\ 
\textbf{ShapeLLM-7B} & 3D Point Cloud & \textbf{-} & - & - & - & - \\
\textbf{ShapeLLM-13B} & 3D Point Cloud & - & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} \\ 
\bottomrule
\end{tabular}
}
\end{table}

==> tab/cls/improvement.tex <==
\begin{table}[t!]
\setlength{\tabcolsep}{6pt}
  \caption{\textbf{Zero-shot 3D multimodal comprehension evaluation} of \textit{core VL capabilities in 3D context} on 3D MM-Vet.
  \textbf{\texttt{Rec}}: General Visual Recognition, \textbf{\texttt{Know}}: Knowledge, \textbf{\texttt{Gen}}: Language Generation, \textbf{\texttt{Spat}}: Spatial Awareness, \textbf{\texttt{Emb}}: Embodied Interaction.
  }
  \label{tab:baseline_imporve}
  \vspace{-5pt}
  \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule[0.95pt]
        Method & \textbf{\texttt{Rec}} & \textbf{\texttt{Know}} & \textbf{\texttt{Gen}} & \textbf{\texttt{Spat}} & \textbf{\texttt{Emb}} & Total  \\ 
        \midrule[0.6pt]
         Point-Bind\&LLM \citep{pointbind23} & 11.3 & 11.6 & 34.2 & 22.2 & 31.9 & 20.0 \\
        PointLLM-7B~\citep{pointllm23} & 32.9 & 25.3 & 33.8 & 31.6 & 26.8 & 29.9 \\
        PointLLM-13B~\citep{pointllm23} & 34.1 & 27.7 & 41.5 & 32.3 & 39.4 & 34.2 \\
        \midrule[0.6pt]
        \rowcolor{linecolor4}\textbf{\shapellm-7B} & \textbf{36.5} & \textbf{33.8} & \textbf{62.0} & \textbf{26.7} & \textbf{71.7} & \textbf{44.2}\\
        \rowcolor{linecolor3}\textbf{\shapellm-13B} & \textbf{42.6} & \textbf{41.2} & \textbf{53.0} & \textbf{38.7} & \textbf{65.2} & \textbf{49.5}\\
        \bottomrule[0.95pt]
    \end{tabular}
    }
\vspace{-8pt}
\end{table}

==> tab/cls/question_num.tex <==
\begin{table}[t!]
  \caption{\textbf{The number of diverse questions} of \textit{core VL capabilities} on 3D MM-Vet
  \texttt{Rec}: General Visual Recognition, \texttt{Know}: Knowledge, \texttt{Gen}: Language Generation, \texttt{Spat}: Spatial Awareness, \texttt{Emb}: Embodied Interaction.
  }
  \label{tab:num}
  \vspace{-5pt}
  \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule[0.95pt]
        \texttt{Rec} & \texttt{Know} & \texttt{Gen} & \texttt{Spat} & \texttt{Emb} & Total  \\ 
        \midrule[0.5pt]
           78 & 76 & 27 & 20 & 39 & 298 \\
        \bottomrule[0.95pt]
    \end{tabular}
    }
\end{table}

==> tab/prompt_num.tex <==
\begin{table}[t!]
  \caption{\textbf{Ablation study on visual prompt number}. The performance of \shapellm\ on 3D MM-Vet is reported.}
  \label{tab:prompt_num}
  \vspace{-5pt}
  \centering
    \resizebox{0.8\linewidth}{!}{
    \begin{tabular}{ccccccc}
    \toprule[0.95pt]
        Number & \textbf{\texttt{Rec}} & \textbf{\texttt{Know}} & \textbf{\texttt{Gen}} & \textbf{\texttt{Spat}} & \textbf{\texttt{Emb}} & Total  \\ 
        \midrule[0.6pt]
        1 &  &  &  &  &  & 51.3 \\
        8 &  &  &  &  &  & 52.2 \\
        16 &  &  &  &  &  & 52.0 \\
        32 &  &  &  &  &  & 53.1 \\
        64 &  &  &  &  &  & 51.9 \\
        \bottomrule[0.95pt]
    \end{tabular}
    }
\end{table}
